Automated Mapping of Vulnerability Advisories onto their Fix Commits in Open Source Repositories

The lack of comprehensive sources of accurate vulnerability data represents a critical obstacle to studying and understanding software vulnerabilities (and their corrections). In this paper, we present an approach that combines heuristics stemming from practical experience and machine-learning (ML) - specifically, natural language processing (NLP) - to address this problem. Our method consists of three phases. First, an advisory record containing key information about a vulnerability is extracted from an advisory (expressed in natural language). Second, using heuristics, a subset of candidate fix commits is obtained from the source code repository of the affected project by filtering out commits that are known to be irrelevant for the task at hand. Finally, for each such candidate commit, our method builds a numerical feature vector reflecting the characteristics of the commit that are relevant to predicting its match with the advisory at hand. The feature vectors are then exploited for building a final ranked list of candidate fixing commits. The score attributed by the ML model to each feature is kept visible to the users, allowing them to interpret the predictions. We evaluated our approach using a prototype implementation named FixFinder on a manually curated data set that comprises 2,391 known fix commits corresponding to 1,248 public vulnerability advisories. When considering the top-10 commits in the ranked results, our implementation could successfully identify at least one fix commit for up to 84.03% of the vulnerabilities (with a fix commit on the first position for 65.06% of the vulnerabilities). In conclusion, our method reduces considerably the effort needed to search OSS repositories for the commits that fix known vulnerabilities.

==> antonino_intro.tex <==
%- OSS is pervasive
%- Impact of vulnerabilities in OSS components can be dramatic
%- Difficult to detect vulnerable components and to assess the impact of their
%vulnerabilities because:
%    - Automated dependency management is often misunderstood
%	- Dependency networks can be large and complex
%	- Metadata may be unreliable
%	- Rebundling
%
%- The most effective method to attack this problem is to adopt a code-based
%  approach (as opposed to high-level metadata about whole binary artifacts or
%  entire products) as the ground truth Mention Steady/Vulas as an example
%- These methods require data about vulnerabilities that includes accurate
%  information about which classes/methods are impacted and how they are fixed.
%
%  - Broaden the scope of the motivation by mentioning the other goal: to have
%comprehensive datasets of fixes to real-world vulnerabilities from which
%researchers can gain insights as to how vulnerabilities happen and how they are
%addressed in practice. This is also the prerequisite for ML-based techniques.
%
%- NOTE: we are focusing here on one motivation (SCA), but we have the other
%one, more general: to have comprehensive datasets of fixes to real-world
%vulnerabilities from which researchers can gain insights as to how
%vulnerabilities happen and how they are addressed in practice. This is also the
%prerequisite for ML-based techniques. Cite work by J Klein (see chat)
%
%\hrule

\section{Introduction}

Over the past two decades, the availability of open-source software (OSS)
components and their adoption have grown so much that the applications that do
not include at least one open-source component are the exception rather than the
norm~\cite{ZaffarKZ11}. OSS components are pervasive in commercial software as
well: 72\% of Fortune 50 companies use GitHub
Enterprise~\cite{github_state_2020}. According to Snyk Technologies~\cite{tal_state_2019}, the large majority of applications on GitHub Enterprise~\cite{github_state_2020} include 10+ open-source components, which
account for as much as 50\% of the entire code-base of those applications.

On the one hand, OSS components have become such an integral part of the large majority of
software (either free or commercial) products, their vulnerabilities can have a
disruptive impact on businesses and on the society at large.

%The effective management of the software supply chain has proven to be a
%critical problem of today's software industry and has received considerable
%attention both from academia and from practitioners.
%

On the other hand, management of a secure software supply chain implies a
vulnerability detection and assessment capability which is years away from maturity; while some approaches (such as Owasp DC \cite{SedekOOK09}) rely on high-level metadata to determine and maintain a mapping between vulnerabilities and the affected artifact, this has shown crucial shortcomings
in practice, such as package dependency management misunderstanding, Dependency networks' complexity, Metadata unreliability, and more. What is more, security issues often appear unpredictably, cause sudden discontinuity and massive impact over critical infrastructure failure, a typical example of which is the recent Sentinel 1 vulnerability manifestation\footnote{\url{https://sentinels.copernicus.eu/web/sentinel/-/copernicus-sentinel-1b-anomaly-update-1}}, which caused critical infrastructure downtime in satellite-based prediction models, from whether prediction to land navigation, and more. In this case, addressing the issue required heavy manual investigation and systems' rework.

At the same time, the most advanced approaches in the research literature use
code-level information about the vulnerable code fragment and its fix; this
enables efficient detection of vulnerable dependencies, as well as accurate
impact assessment through reachability analysis~\cite{ponta_emse_2020}. Unfortunately, such research relies on data about security vulnerabilities which is scattered across
heterogeneous repository sources, often not machine-readable, and does not provide the
the necessary level of detail, especially when it comes to code-level details, with manual approaches~\cite{ponta_manually-curated_2019} to find such
data being unscalable proportionally to the amount of open-source code developed by
the community and incorporated in commercial products.

Consequently, the role of automated tools becomes vital~\cite{sabetta_practical_2018,CabreraLozoya2021}. Academic and industrial researchers have mostly focused on the classification of
security-relevant commits, where a critical piece of data is the commit that
introduces or fixes \emph{a specific} vulnerability. However, this kind of research
requires a large amount of training data to be available, which leads to a
somewhat circular problem and makes it near impossible to have
comprehensive datasets of fixes to real-world vulnerabilities from which
researchers can gain insights as to how vulnerabilities happen and how they are
addressed in practice. This is a critical prerequisite for more intelligent security and vulnerability analysis mechanisms, e.g., featuring ML-based techniques \cite{klein}.

To this aim, we propose an approach consisting of three sequential steps:
\textbf{(1)}~\emph{extract} - a record containing all relevant vulnerability
information is created from the heterogeneous vulnerability data;
\textbf{(2)}~\emph{filter} - this \emph{advisory record} is used select
candidate commits by filtering out those that, based on heuristics motivated by
observations on the available vulnerability data, are known to be irrelevant for
the task at hand; \textbf{(3)}~\emph{rank} - these candidate commits are ranked
based on their probability of being a fix commit \emph{for the advisory record}
given as input.

In this paper, we present a prototype (named \prospector) that implements
our method. \prospector provides a proof-of-concept that can serve as a baseline
for further experimentation and research as well as for the implementation of a
usable solution to be adopted in an industrial context. \prospector is released
as open-source software as part of SAP's \textsc{project
    ``KB''}\footnote{\url{https://github.com/sap/project-kb}}, whose goal is to
\emph{support the creation, management, and aggregation of a distributed,
    collaborative knowledge base of vulnerabilities that affect open-source
    software}.

To the best of our knowledge, no similar research has been done in the current
state of the literature in the security engineering research domain, most of the
existing related research has rather focused on the related but distinct problem
of predicting whether a commit introduces or fixes \emph{some} vulnerability.
The problem of determining whether a commit is the fix commit \emph{for a
    specific vulnerability} (as described in an advisory) has not received much
attention from the research community, despite being of practical relevance.

Our experimentation with \prospector shows that this method can identify
the fix commits of an advisory with a precision of \rankingprecision{}\% and a
recall in the top ten (\rankingrecallten{}\%). This performance makes the tool
suitable for practical use in that it allows the effort of the human expert to
be dedicated to the (relatively few) residual cases that the tool could not deal
with.

The remainder of the paper is organized as follows. In~\Cref{motivation}, we
provide background information and elaborate on the need for a method to
automate the process of finding fix commits for known vulnerabilities in OSS.
\Cref{description} describes the three pillars of the approach; our
implementation of this method is presented in \Cref{implementation}. The
evaluation of our method is presented in \Cref{evaluation}. In
\Cref{discussion}, we elaborate on the findings gathered from our experiment,
and we outline opportunities for further research. After a brief overview
of the current state of the literature is given in \Cref{related_work},
\Cref{conclusion} concludes the paper.


==> intro-revised.tex <==
%- OSS is pervasive
%- Impact of vulnerabilities in OSS components can be dramatic
%- Difficult to detect vulnerable components and to assess the impact of their
%vulnerabilities because:
%    - Automated dependency management is often misunderstood
%	- Dependency networks can be large and complex
%	- Metadata may be unreliable
%	- Rebundling
%
%- The most effective method to attack this problem is to adopt a code-based
%  approach (as opposed to high-level metadata about whole binary artifacts or
%  entire products) as the ground truth Mention Steady/Vulas as an example
%- These methods require data about vulnerabilities that includes accurate
%  information about which classes/methods are impacted and how they are fixed.
%
%  - Broaden the scope of the motivation by mentioning the other goal: to have
%comprehensive datasets of fixes to real-world vulnerabilities from which
%researchers can gain insights as to how vulnerabilities happen and how they are
%addressed in practice. This is also the prerequisite for ML-based techniques.
%
%- NOTE: we are focusing here on one motivation (SCA), but we have the other
%one, more general: to have comprehensive datasets of fixes to real-world
%vulnerabilities from which researchers can gain insights as to how
%vulnerabilities happen and how they are addressed in practice. This is also the
%prerequisite for ML-based techniques. Cite work by J Klein (see chat)
%
%\hrule

\section{Introduction}

Over the past two decades, the availability of open-source software (OSS)
components and their adoption have grown so much that the applications that do
not include at least one open-source component are the exception rather than the
norm~\cite{ZaffarKZ11}. OSS components are pervasive in commercial software as
well: 72\% of Fortune 50 companies use GitHub
Enterprise~\cite{github_state_2020}. According to Snyk Technologies~\cite{tal_state_2019}, the large majority of applications on GitHub Enterprise~\cite{github_state_2020} include 10+ open-source components, which
account for as much as 50\% of the entire code-base of those applications.

On the one hand, OSS components have become such an integral part of the large majority of
software (either free or commercial) products, their vulnerabilities can have a
disruptive impact on businesses and on the society at large.

%The effective management of the software supply chain has proven to be a
%critical problem of today's software industry and has received considerable
%attention both from academia and from practitioners.
%

On the other hand, management of a secure software supply chain implies a
vulnerability detection and assessment capability which is years away from maturity; while some approaches (such as Owasp DC \cite{SedekOOK09}) rely on high-level metadata to determine and maintain a mapping between vulnerabilities and the affected artifact, this has shown crucial shortcomings
in practice, such as package dependency management misunderstanding, Dependency networks' complexity, Metadata unreliability, and more. What is more, security issues often appear unpredictably, cause sudden discontinuity and massive impact over critical infrastructure failure, a typical example of which is the recent Sentinel 1 vulnerability manifestation\footnote{\url{https://sentinels.copernicus.eu/web/sentinel/-/copernicus-sentinel-1b-anomaly-update-1}}, which caused critical infrastructure downtime in satellite-based prediction models, from whether prediction to land navigation, and more. In this case, addressing the issue required heavy manual investigation and systems' rework.

At the same time, the most advanced approaches in the research literature use
code-level information about the vulnerable code fragment and its fix; this
enables efficient detection of vulnerable dependencies, as well as accurate
impact assessment through reachability analysis~\cite{ponta_emse_2020}. Unfortunately, such research relies on data about security vulnerabilities which is scattered across
heterogeneous repository sources, often not machine-readable, and does not provide the
the necessary level of detail, especially when it comes to code-level details, with manual approaches~\cite{ponta_manually-curated_2019} to find such
data being unscalable proportionally to the amount of open-source code developed by
the community and incorporated in commercial products.

Consequently, the role of automated tools becomes vital~\cite{sabetta_practical_2018,CabreraLozoya2021}. Academic and industrial researchers have mostly focused on the classification of
security-relevant commits, where a critical piece of data is the commit that
introduces or fixes \emph{a specific} vulnerability. However, this kind of research
requires a large amount of training data to be available, which leads to a
somewhat circular problem and makes it near impossible to have
comprehensive datasets of fixes to real-world vulnerabilities from which
researchers can gain insights as to how vulnerabilities happen and how they are
addressed in practice. This is a critical prerequisite for more intelligent security and vulnerability analysis mechanisms, e.g., featuring ML-based techniques \cite{klein}.

To this aim, we propose an approach consisting of three sequential steps:
\textbf{(1)}~\emph{extract} - a record containing all relevant vulnerability
information is created from the heterogeneous vulnerability data;
\textbf{(2)}~\emph{filter} - this \emph{advisory record} is used select
candidate commits by filtering out those that, based on heuristics motivated by
observations on the available vulnerability data, are known to be irrelevant for
the task at hand; \textbf{(3)}~\emph{rank} - these candidate commits are ranked
based on their probability of being a fix commit \emph{for the advisory record}
given as input.

In this paper, we present a prototype (named \prospector) that implements
our method. \prospector provides a proof-of-concept that can serve as a baseline
for further experimentation and research as well as for the implementation of a
usable solution to be adopted in an industrial context. \prospector is released
as open-source software as part of SAP's \textsc{project
    ``KB''}\footnote{\url{https://github.com/sap/project-kb}}, whose goal is to
\emph{support the creation, management, and aggregation of a distributed,
    collaborative knowledge base of vulnerabilities that affect open-source
    software}.

To the best of our knowledge, no similar research has been done in the current
state of the literature in the security engineering research domain, most of the
existing related research has rather focused on the related but distinct problem
of predicting whether a commit introduces or fixes \emph{some} vulnerability.
The problem of determining whether a commit is the fix commit \emph{for a
    specific vulnerability} (as described in an advisory) has not received much
attention from the research community, despite being of practical relevance.

Our experimentation with \prospector shows that this method can identify
the fix commits of an advisory with a precision of \rankingprecision{}\% and a
recall in the top ten (\rankingrecallten{}\%). This performance makes the tool
suitable for practical use in that it allows the effort of the human expert to
be dedicated to the (relatively few) residual cases that the tool could not deal
with.

The remainder of the paper is organized as follows. In~\Cref{motivation}, we
provide background information and elaborate on the need for a method to
automate the process of finding fix commits for known vulnerabilities in OSS.
\Cref{description} describes the three pillars of the approach; our
implementation of this method is presented in \Cref{implementation}. The
evaluation of our method is presented in \Cref{evaluation}. In
\Cref{discussion}, we elaborate on the findings gathered from our experiment,
and we outline opportunities for further research. After a brief overview
of the current state of the literature is given in \Cref{related_work},
\Cref{conclusion} concludes the paper.


==> tables/nvd_reference_analysis.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|ll}
    \toprule
         \textbf{Method}        & \textbf{Known fix commits found (\%)} & \textbf{A fix found for CVEs (\%) }   \\
     \hline
    \midrule
         CVE ID in message      &  19.20                                & 12.18                                 \\
         Referred by the NVD    &  7.53                                 & 11.46                                 \\                 
         Jimenez et al.         &  26.06                                & 22.36                                 \\
    \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Results of the NVD reference analysis. For all known fix commits in the data set, it is explored whether the commit mentions the CVE ID in the commit message, or the NVD-page of the vulnerability refers to the commit.}
    \label{tab:nvd_reference_analysis}
\end{table}

==> tables/ranking_results.tex <==
% \begin{table}[!h]
%     \centering
%     \begin{small}
%         \begin{tabular}{lllllll}
%         \toprule
%               &     & precision & avg. pos. &    recall at 5 &   recall at 10 &   recall at 20 \\
%         split & model &               &                     &                &                &                \\
%         \midrule
%         test  & AB &   62.67 (2.5) &        24.25 (8.86) &   75.89 (2.81) &   83.26 (2.13) &    87.68 (2.1) \\
%               & KNNC &  18.04 (9.38) &       108.65 (35.5) &  27.13 (15.24) &  39.22 (14.86) &   54.7 (12.55) \\
%               & LR &  \textbf{65.06 (1.91)} &        22.89 (5.47) &   \textbf{77.68 (1.41)} &   \textbf{84.03 (1.22)} &    \textbf{88.24 (1.0)} \\
%               & RF &  56.77 (1.96) &         \textbf{18.5 (4.81)} &   73.13 (1.39) &   81.54 (1.58) &   87.58 (1.81) \\
%               & SVC &  61.89 (5.44) &        22.48 (5.83) &   75.72 (3.65) &   82.64 (2.65) &   87.37 (2.31) \\
%         train & AB &    64.5 (1.0) &        15.12 (2.33) &    78.0 (1.18) &   84.76 (0.52) &   89.51 (0.42) \\
%               & KNNC &  21.46 (9.02) &        34.98 (9.95) &   32.1 (13.56) &  44.59 (14.66) &  60.88 (12.56) \\
%               & LR &  65.33 (0.94) &        21.16 (2.37) &    78.26 (0.7) &   85.11 (0.53) &   89.38 (0.42) \\
%               & RF &  79.94 (1.49) &         1.62 (0.16) &   91.84 (0.84) &    95.97 (0.6) &   98.23 (0.44) \\
%               & SVC &  62.36 (4.49) &         19.88 (2.1) &     76.3 (3.2) &   83.49 (1.93) &   89.35 (0.66) \\
%         \bottomrule
%         \end{tabular}
%     \end{small}
    
%     \caption{The performance of the different machine learning algorithms on ranking the candidate commits after applying a combination of vulnerability specific and universal scaling (standard deviation denoted between parentheses).}
%     \label{tab:ranking_results_all_components_scaling_combination}
% \end{table}

\begin{table}
    \centering
    \begin{small}
        \begin{tabular}{l|llllll}
        \textbf{split} & \textbf{model} & \textbf{precision}             & \textbf{avg. pos.}         &    \textbf{recall at 5} &   \textbf{recall at 10} &   \textbf{recall at 20} \\
        \hline
        \midrule
        test  & AB      & 62.67 (2.5)           & 24.25 (8.86)      &   75.89 (2.81) &   83.26 (2.13) &    87.68 (2.1) \\
              & KNNC    & 18.04 (9.38)          & 108.65 (35.5)     &  27.13 (15.24) &  39.22 (14.86) &   54.7 (12.55) \\
              & LR      & \textbf{65.06 (1.91)} & 22.89 (5.47)      &   \textbf{77.68 (1.41)} &   \textbf{84.03 (1.22)} &    \textbf{88.24 (1.0)} \\
              & RF      & 56.77 (1.96)          & \textbf{18.5 (4.81)} &   73.13 (1.39) &   81.54 (1.58) &   87.58 (1.81) \\
              & SVC     & 61.89 (5.44)          & 22.48 (5.83)      &   75.72 (3.65) &   82.64 (2.65) &   87.37 (2.31) \\
        \hline
        train & AB      & 64.5 (1.0)            & 15.12 (2.33)      &    78.0 (1.18) &   84.76 (0.52) &   89.51 (0.42) \\
              & KNNC    & 21.46 (9.02)          & 34.98 (9.95)      &   32.1 (13.56) &  44.59 (14.66) &  60.88 (12.56) \\
              & LR      & 65.33 (0.94)          & 21.16 (2.37)      &    78.26 (0.7) &   85.11 (0.53) &   89.38 (0.42) \\
              & RF      & 79.94 (1.49)          & 1.62 (0.16)       &   91.84 (0.84) &    95.97 (0.6) &   98.23 (0.44) \\
              & SVC     & 62.36 (4.49)          & 19.88 (2.1)       &     76.3 (3.2) &   83.49 (1.93) &   89.35 (0.66) \\
        \bottomrule
        \end{tabular}
        \vspace{3mm}
    \end{small}
    
    \caption{The performance of the different machine learning algorithms on ranking the candidate commits after applying a combination of vulnerability specific and universal scaling (standard deviation denoted between parentheses).}
    \label{tab:ranking_results_all_components_scaling_combination}
\end{table}
